This Looks Better than That: Better Interpretable Models with ProtoPNeXt

Prototypical-part models are a popular interpretable alternative to black-box deep learning models for computer vision. However, they are difficult to train, with high sensitivity to hyperparameter tuning, inhibiting their application to new datasets and our understanding of which methods truly improve their performance. To facilitate the careful study of prototypical-part networks (ProtoPNets), we create a new framework for integrating components of prototypical-part models -- ProtoPNeXt. Using ProtoPNeXt, we show that applying Bayesian hyperparameter tuning and an angular prototype similarity metric to the original ProtoPNet is sufficient to produce new state-of-the-art accuracy for prototypical-part models on CUB-200 across multiple backbones. We further deploy this framework to jointly optimize for accuracy and prototype interpretability as measured by metrics included in ProtoPNeXt. Using the same resources, this produces models with substantially superior semantics and changes in accuracy between +1.3% and -1.5%. The code and trained models will be made publicly available upon publication.

==> archive/abstract_drafts.tex <==
Prototypical part models are an interpretable alternative to black-box deep learning models. However, they have proven difficult to train, require difficult hyperparameter tuning when deployed to new datasets, and suffer from complex and inconsistent code. 
We address these problems by constructing a modular framework for prototypical part models -- called ProtoPNext -- that directly integrates Bayesian hyperparameter tuning, interpretability metrics, and features from multiple prototypical models. 
We show that, with minimal methodological changes, our framework allows us to produce models that exceed state-of-the-art accuracy on CUB200 across multiple backbones. 
Using ProtoPNext's built-in interpretability metrics, we demonstrate that optimizing directly for prototype interpretability can improve interpretability over multiple metrics with negligible cost to accuracy. 
%Finally, we show that these models can leverage modern backbones like ConvNeXt to further advance the state of the art. 

%%% Drafting

% We address these problems by constructing a modular framework for prototypical part models -- called ProtoPNext -- that directly integrates Bayesian hyperparameter tuning, interpretability metrics, and features from multiple prototypical models.
% We show that, with minimal methodological changes, our framework allows us to produce models that exceed state-of-the-art accuracy on CUB200 across multiple backbones. Using ProtoPNext's built in interpretability metrics, we demonstrate that optimizing directly for prototype interpretability can improve interpretability over multiple metrics with negligible cost to accuracy.


% Prototypical part models are an interpretable alternative to black-box deep learning models. However, they have proven difficult to train. In this work, we show that by replacing only the L2 distance metric used by Chen et al. to assess prototype similarity with a Cosine similarity metric, we can dramatically improve convergence rates and reduce computational code by over an order of magnitude. Using this computational advantage, we optimize ProtoPNet models, establishing new states of the art on CUB200 over multiple backbones. We further leverage the larger candidate model set to demonstrate optimizing directly for prototype interpretability can improve interpretability over multiple metrics at less than a 1\% cost in accuracy. Finally, we show that these cosine models can leverage modern backbones like ConvNeXt to further advance the state of the art.

% However, they have proven difficult to train with high sensitivity to hyperparameter tuning, limiting their application to new datasets and novel applications.

%We present ProtoPNeXt, an improvement to the popular ProtoPNet algorithm released by Chen et al. in 2019. 
%The original algorithm uses case-based reasoning on image parts to provide interpretable image classification while maintaining the performance improvements provided by deep neural network models and pretraining. 
%Improvements in ProtoPNeXt include dramatically increased performance, reduced reliance on manual hyperparameter tuning, a unified framework that combines improvements from disparate prototypical-part models, easier to use code, and a suite of built-in interpretability and analysis tools. 
%The code base is publicly available at \textit{$<$url omitted for blind review$>$}.
%Across three case studies using capabilities integrated into ProtoPNeXt, we 
%1) create novel prototypical-part models that source aspects of previous models, the combination exceeding the performance of any of the source models; 
%2) reduce inequality in racial-subgroup performance for an interpretable breast cancer diagnosis model; 
%3) using the same GPU resources, we produce xx\% more models that are interpretable during a hyperparameter sweep because we optimize for both accuracy and interpretability metrics.

==> archive/case_study_2.tex <==
Our new framework readily supports subgroup analysis during training and validation. This enables direct tuning for desired fairness metrics, such as equal predictive power for different racial subgroups for medical image analysis.

In this case study, we demonstrate how the new system can lead to a model selection with better fairness outcomes. Using a dataset where each patient is labelled according to their racial subgroup, we conduct two hyperparameter sweeps. The first incorporates the subgroup fairness metric ---- introduced by ---et al. in -----. The second includes no subgroup analysis during tuning. 

%results go here

While it may seem trivial that tuning for fairness metrics results in fairer models, in previous studies using the ProtoPNet backbone to evaluate medical datasets, subgroup analysis was 
only performed after model selection (papers ----) %IAIA-BL ext val
or not at all (papers -----). %IAIA-BL NMI, NEJM AI EEG paper, 

==> archive/design_principles.tex <==
\subsection{Design Principles}
\label{subsec:design_principles}
Our top priority in designing ProtoPNext was ease of use, both for practitioners and future researchers. This motivates us to follow three primary design principles:

\textbf{First-Class Prototypes.} Models built with ProtoPNeXt have prototypes as first-class citizens. Non-gradient-based prototype training steps are natively supported and metadata about prototypes is available through an intuitive interface. ProtoPNeXt includes visualization components that make it easy to visualize the relationships between model predictions and the prototypes that yield those those predictions.

\textbf{Use PyTorch Whenever Possible.} The machine learning community has widely adopted PyTorch \cite{paszke2019pytorch} as the de facto framework for deep learning models. ProtoPNext is built on top of native PyTorch, and follows idiomatic PyTorch design whenever possible. Training in ProtoPNeXt uses PyTorch's autograd and backpropagation for gradient-based updates, and training and inference both take advantage of accelerators via PyTorch's standard interface.
Aside from the prototype-specific components that ProtoPNeXt adds, ProtoPNeXt should be immediately familiar to the whole deep learning community.

\textbf{Modularity and Extensibility.} In ProtoPNext, core components of the case-based DNN into distinct torch modules that are composed to make a new network. ProtoPNeXt defines semantics for a Prototypical Part Network and its prototypes with out-of-the-box implementations, but is ultimately implementation agnostic. By doing so, we make it simple to extend and replace individual network components with others from existing and new architectures, with the goal of accelerating the development of new case-based architectures.

% \textbf{Extensibility} A key goal of this framework is to support and accelerate the development of future case-based DNN methods. As such, the framework needs to readily accommodate new modules. We accomplished this by ...
With our design goals detailed, we now turn to formally introduce ProtoPNet \cite{chen2019looks} as it is implemented in ProtoPNext.


==> archive/title-ideas.tex <==
% ProtoPNeXt: modern, user-friendly tools for better prototypical-part networks
% ProtoPNeXt: A usuable prototypical-part network
% ProtoPNeXt: Prototype model for Pytorch
% ProtoPNeXt: Improved tools for traning and evaluating prototypical-part networks
% ProtoPNeXt: User-friendly tools for better prototypical-part networks
% ProtoPNeXt: Modern, user-friendly tools for better prototypical-part networks
% ProtoPNeXt: Modern prototypical-part networks for user-friendliness
% ProtoPNeXt: Interpretability-first for prototypical-part networks
% ProtoPNeXt: Training interpretable models for interpretability
% ProtoPNeXt: Training prototypical-part networks for interpretability
% Making it easier to build interpretable models with ProtoPNeXt
% Making interpretable models with ease using ProtoPNeXt
% Bulding interpretable model with ease using ProtoPNeXt
% Easy Interpretable Model Development with ProtoPNeXt
% Practioner-friendly Interpretable Model Development with ProtoPNeXt
% Rapidly develop better interpretable models with ProtoPNeXt
% Building better interpretables model easily using ProtoPNeXt
% Pythonic Interpretable Model Development with ProtoPNeXt
% Easily develop better interpretable models with ProtoPNeXt


==> author_cont.tex <==
[Removed for anonymization.]

==> tables/joint-extended.tex <==
\begin{tabular}{lllllllll}
\toprule
 & densenet121 & resnet34 & vgg16 & convnext-l-22k & convnext-b-22k & vgg19 & densenet161 & resnet50 \\
\midrule
\bottomrule
\end{tabular}


==> tables/l2-full-acc.tex <==
\begin{tabular}{llllllll}
\toprule
 & backbone & DenseNet-121 & DenseNet-161 & ResNet-34 & ResNet-50 & VGG-16 & VGG-19 \\
arch & distance &  &  &  &  &  &  \\
\midrule
deformable & cos & 75.4 & 79.1 & 73.6 & 85.5 & 74.4 & 74.0 \\
\cline{1-8}
\multirow[t]{2}{*}{vanilla} & cos & 75.5 & 80.7 & 74.4 & 86.4 & 74.2 & 74.1 \\
 & l2 & nan & nan & nan & nan & nan & 68.8 \\
\cline{1-8}
\bottomrule
\end{tabular}

